Learning to design protein-protein interactions with enhanced generalization

Discovering mutations enhancing protein-protein interactions (PPIs) is critical for advancing biomedical research and developing improved therapeutics. While machine learning approaches have substantially advanced the field, they often struggle to generalize beyond training data in practical scenarios. The contributions of this work are three-fold. First, we construct PPIRef, the largest and non-redundant dataset of 3D protein-protein interactions, enabling effective large-scale learning. Second, we leverage the PPIRef dataset to pre-train PPIformer, a new SE(3)-equivariant model generalizing across diverse protein-binder variants. We fine-tune PPIformer to predict effects of mutations on protein-protein interactions via a thermodynamically motivated adjustment of the pre-training loss function. Finally, we demonstrate the enhanced generalization of our new PPIformer approach by outperforming other state-of-the-art methods on new, non-leaking splits of standard labeled PPI mutational data and independent case studies optimizing a human antibody against SARS-CoV-2 and increasing the thrombolytic activity of staphylokinase.

==> assets/fig_pre-training_ablations.tex <==
\begin{wrapfigure}{R}{9cm}

\vspace{-20pt}

\ffigbox[\textwidth]
{
    \caption{Pre-training ablations with respect to datasets and \ppiformer masking strategies, input protein representations, and loss functions. The metrics show zero-shot performance on the training fold of the SKEMPI v2.0 dataset, i.e. $\Delta \Delta G$ inference according to \Cref{eq:ddg-pred} without any supervision. Each row in the figure represents a single modification of the complete \ppiformer model.
    Dataset ablations precede model ablations, using different SKEMPI v2.0 subsets. The former evaluated on two of three folds by \citep{luo2023rotamer}, and the latter on the training set from the split described in \Cref{sec:eval-data}. Thus, performance varies slightly between (a3) and \ppiformer rows, despite representing the same model.}
}
{
    \label{fig:ablations}
    \includegraphics[width=\textwidth]{assets/pre-training_ablations.pdf}
}

\vspace{-20pt}

\end{wrapfigure}


==> assets/fine-tuning-ablation.tex <==
\begin{wrapfigure}{R}{4cm}

\vspace{-0.55cm}

\ffigbox[\textwidth]
{
    \caption{The effect of pre-training on $\Delta \Delta G$ fine-tuning. A training step is performed by sampling a single mutation from each PPI in a randomly sampled batch. The shaded areas correspond to the minimum, mean and maximum of the performance of three models on three-fold cross-validation.
    }
}
{
    \label{fig:pretraing-helps}
    \includegraphics[width=\textwidth]{assets/pre-trianing_vs_no_pre-training.pdf}
}

\vspace{-1cm}

\end{wrapfigure}
